Incremental Database Design using UML-B and Event-B

Correct operation of many critical systems is dependent on the data consistency and integrity properties of underlying databases. Therefore, a verifiable and rigorous database design process is highly desirable. This research aims to investigate and deliver a comprehensive and practical approach for modelling databases in formal methods through layered refinements. The methodology is being guided by a number of case studies, using abstraction and refinement in UML-B and verification with the Rodin tool. UML-B is a graphical representation of the Event-B formalism and the Rodin tool supports verification for Event-B and UML-B. Our method guides developers to model relational databases in UML-B through layered refinement and to specify the necessary constraints and operations on the database.

==> eptcsdata.tex <==
\providecommand{\firstpage}{34}
\providecommand{\publicationstatus}{R. Laleau, D. M\'ery, S. Nakajima, E. Troubitsyna (Eds): Joint Workshop on\\ Handling IMPlicit and EXplicit knowledge in formal system development\\ and  Formal \& Model-Driven Techniques for Developing Trustworthy Systems.\\
EPTCS 271, 2018, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.271.3}{10.4204/EPTCS.271.3}}
\pdfoutput=1

